Behaviorally Diverse Traffic Simulation via Reinforcement Learning

Traffic simulators are important tools in autonomous driving development. While continuous progress has been made to provide developers more options for modeling various traffic participants, tuning these models to increase their behavioral diversity while maintaining quality is often very challenging. This paper introduces an easily-tunable policy generation algorithm for autonomous driving agents. The proposed algorithm balances diversity and driving skills by leveraging the representation and exploration abilities of deep reinforcement learning via a distinct policy set selector. Moreover, we present an algorithm utilizing intrinsic rewards to widen behavioral differences in the training. To provide quantitative assessments, we develop two trajectory-based evaluation metrics which measure the differences among policies and behavioral coverage. We experimentally show the effectiveness of our methods on several challenging intersection scenes.

==> sec-reference-trajectory-generation.tex <==
\section{Reference Trajectory Generation} \label{sec: reference trajectory generation}

In our experiment, we modeled reference trajectories for an intersection scene as a \emph{Brownian bridge}
bent along some desired trajectory named \emph{core trajectory},
with the conversion by a P-control agent to consider the dynamics and surroundings.
Details of parameters used in experiments are shown in Section \ref{subsec: experimental setting}.

\subsection{Brownian bridge trajectory generation} \label{subsec: single_bb}
To generate diverse trajectories, we first define a \emph{core trajectory}, an expected average trace, and then perturb it with longitudinal and lateral movements along with it.
For lateral movements, we applied a Brownian bridge whose variance is $\sigma_\text{(la)}$.
For longitudinal movements, we set its speed along the core trajectory by a Brownian bridge of the variance $\sigma_\text{(lo)}$ with adding a constant speed $v_\text{(lo)}$.

\subsection{Trajectory conversion considering vehicle dynamics}

We also implement a converter from the trajectories of Brownian bridges shown in \ref{subsec: single_bb} trajectories to ones considering obstacles and vehicle dynamics.

For dynamics, we replaced the original trajectories by trajectories generated by a P-control agent mimicking them.
Let $p^{original}$ and $p$ denote the original trajectory and the converted one. Then the P-control agent at time $t$ will try to move from point $p(t)$, in two seconds, to the target point $p^{target}(t) = p^{original}(t+2)$ which is the point in the original trajectory in two seconds later.
More precisely, the steering angle $\phi_t$ (rad) and the acceleration $a_t$ ($\mathrm{m/s^2}$) are defined as follows:
\begin{itemize}
    \item $\phi_t = w_\phi \cdot \sin{\omega}$ where $w_\phi$ is the weight coefficient and $\omega$ is the angle difference.
    \item $a_t =  w_a \cdot \frac{|p^\text{target}(t) - p(t)|}{2} - v(t)\sin{\omega}$ where $w_a$ is the weight coefficient and $v(t)$ is the current speed.
\end{itemize}
We set $(w_\phi, w_a) = (1.0, 3.0)$ in our experiments. %

For obstacles, the conversion is done in a straight-forward way:  %
run the agent without looking at any obstacles and apply the trajectory if the agent reached the goal without collision.
Fig. \ref{fig:reference_trajectory} describes an example of the converted trajectory set in one scenario.



